Observationally Cooperative Multithreading

Despite widespread interest in multicore computing, concur- rency models in mainstream languages often lead to subtle, error-prone code. Observationally Cooperative Multithreading (OCM) is a new approach to shared-memory parallelism. Programmers write code using the well-understood cooperative (i.e., nonpreemptive) multithreading model for uniprocessors. OCM then allows threads to run in parallel, so long as results remain consistent with the cooperative model. Programmers benefit because they can reason largely sequentially. Remaining interthread interactions are far less chaotic than in other models, permitting easier reasoning and debugging. Programmers can also defer the choice of concurrency-control mechanism (e.g., locks or transactions) until after they have written their programs, at which point they can compare concurrency-control strategies and choose the one that offers the best performance. Implementers and researchers also benefit from the agnostic nature of OCM -- it provides a level of abstraction to investigate, compare, and combine a variety of interesting concurrency-control techniques.

==> Makefile <==
DIAGRAMS = 
TEX_PARTS = abstract.tex conclusions.tex debugging.tex \
	    implementation.tex background-alt.tex \
            intro.tex macros.tex motivation.tex ocm.tex oursolution.tex \
            performance.tex relatedwork.tex semantics.tex ocm.bib \
            relatedwork-alt.tex ants.tex \
            perf-fig1.tex perf-fig2.tex


include Makefile.$(shell uname -s)

all: ocm.pdf

ocm.pdf: $(TEX_PARTS) $(DIAGRAMS)
	pdflatex ocm
	bibtex ocm
	pdflatex ocm
	pdflatex ocm

%.pdf: %.eps
	$(CONVERT_EPS2PDF) $<

clean:
	rm -f ocm.pdf ocm.aux ocm.bbl ocm.blg ocm.dvi ocm.log
	rm -f $(DIAGRAMS)


==> grant_proposal.tex <==
%!TEX root = ocm.tex

\section{GRANT PROPOSAL} 
The trend towards multicore CPUs is well under way; 8 to 16 cores per
chip will be widely available in the next few years, and 128-core CPUs
are already under development. Modern graphics cards already have
hundreds of processing units, which are becoming more and more general
purpose. With several multicore CPUs on one motherboard,
the average desktop computer will have immense processing power.

Unfortunately, programmers already struggle to take full advantage of
multiple processors. Decades of experience has shown that it is
surprisingly difficult to write correct sequential
code;\footnote{``By June 1949, people had begun
  to realize that it was not so easy to get a program right as it had at
  one time appeared\ldots{}  It was on one of my journeys between the EDSAC
  room and the punching equipment that \ldots the realization came over
  me with full force that a good part of the remainder of my life was
  going to be spent in finding errors in my own
  programs.''~\citet{Wilkes:85:mmrs-cmptr:book}}.%
\textsuperscript{,}\footnote{``I was amazed: given ample time, only about ten
  percent of professional programmers were able to get [binary search]
right.'' \citet{Bentley:86:prgrmmng-prls:book}.}%
\textsuperscript{,}\footnote{``Fast forward to 2006. I was shocked to learn that the
  binary search program that Bentley proved correct and subsequently
  tested in Chapter 5 of Programming Pearls contains a bug\ldots The
  general lesson that I take away from this bug is humility: It is
  hard to write even the smallest piece of code correctly, and our
  whole world runs on big, complex pieces of code.'' ~\citet{Bloch:06:extr-extr:unpub}.}
concurrent
programs can be far more difficult. All the problems of sequential
code remain, combined with race conditions, deadlock, and
nondeterminism.

If there is only a handful of simultaneous threads of execution to
worry about, then traditional facilities in mainstream languages
(e.g., preemptive threads, and locks or monitors) can be made to work,
given enough extra care while programming.  Conversely, huge numbers of
threads are no problem if they are independent and noninteracting
(e.g., GPU shaders). But few applications are so embarrassingly
parallel, while a handful of threads cannot make good use of a hundred
cores.


Tim Sweeney, founder of Epic Games, described a typical situation in his
industry: game state consists of thousands of mutable objects, each
object is updated many times per second, and each update involves a
handful of other objects~\citep{Sweeney:06:nxt-mnstrm:popl}.  As a consequence,
most updates are independent of one another, but not all, and
interactions between objects change rapidly as the game
progresses. It would make sense---both for better code structure and
for exploiting multiprocessors---to divide this work into as many
threads as
one per game object, but in any mainstream language the sheer
complexity of synchronization between threads would be overwhelming.


%\cas{Andrew suggests mentioning something about MPI and other
%``most successful'' uses of threads. I don't really have anything
%useful to say. Do you?}

Taking real advantage of future hardware thus relies on finding better
ways to write concurrent code.  In light of modern implementation
techniques, we believe it is time to reevaluate the cooperative
(nonpreemptive) model of multithreading for shared-memory concurrency
on multiprocessors.  Specifically, we propose \keyterm{\OCM (OCM)}, a
system where programmers write and reason about code as if
one thread runs at a time until it explicitly yields control, but
which actually runs many threads simultaneously on separate processors,
possibly even switching preemptively.

In the following sections, we summarize the advantages of cooperative
multithreading, describe OCM more specifically, and outline our
research plans.



% \section{Preemptive Multitasking and Cooperative Multithreading}
\section{Threading and Synchronization Models}


\iffalse
We therefore propose to reevaluate the cooperative multithreading
model in the light of new implementation techniques.  We are
developing \textbf{\OCM (OCM)}, a system in which programmers can
reason about code as if one thread runs at a time, but with an
underlying implementation that runs many threads simultaneously and
schedules them preemptively.

OCM is inspired by the Automatic Mutual Exclusion approach to
Transactional Memory.  But AME builds a language around transactions,
resulting in a language reminiscent of cooperative multithreading. In
contrast, we propose to start from the cooperative
model, and then use all available techniques to achieve an efficient
and practical multiprocessor implementation.
\fi

\iffalse
Taking real advantage of future architectures thus relies on finding
better ways to write concurrent code.  There have been many proposals
over the span of decades, but one of the most intriguing recent
suggestions is Transactional
Memory~\citep{Harris-et-al:05:cmpsbl-mmry:ppopp,Larus-Rajwar:07:trnsctnl-mmry:slca}.  By taking atomic
transactions as a primitive operation, concurrent code can avoid
complex inter-thread synchronization. Many of the traditional
difficulties with locks are be avoided.

The potential benefits of Transactional Memory are tantalizing, but
the actual practicality and scalability has yet to be convincingly
demonstrated.  There are few examples of large systems using TM, and
few of these were written from scratch (as opposed to being adapted
from code already structured around explicit locking and
synchronization).

In contrast, there is already strong evidence for
cooperative multithreading as an intuitive model. Large systems have
been written quite successfully using cooperative multithreading
\cas{Examples?}, and because cooperative thread systems were often
lightweight, some of these systems involved very large numbers of
threads. \cas{Is this true?}
\fi


\noindent
To explore the issues that exist with traditional parallel programming, we will show and develop a simple and familiar example in which we transfer funds between bank accounts.

Assume that we have the following two threads of control:
{\columnseprule=0.4pt

\begin{multicols}{2}
  \begin{Verbatim}
   // Send $5.00 from src to dst1
   src  = src - 5;
   dst1 = dst1 + 5;
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     // Send $10.00 from src to dst2
     src  = src - 10;
     dst2 = dst2 + 10;
\end{Verbatim}
\end{multicols}
}

\subsection{Traditional Preemptive Multitasking with Locks}


In the preemptive model familiar from \Java threads or \Unix \Pthreads,
multiple threads may execute simultaneously and/or we can switch between
different threads at unpredictable times.  Once both
threads here have terminated, we might expect that \cTX{src} has decreased
by \cTX{\$15}.  But in this traditional model, the code has race conditions.
For example, in some possible executions, \cTX{src} could decrease by only
\cTX{\$5} or \cTX{\$10} (if the second thread executed in its entirety between the
first thread's read of \cTX{src} and its write to \cTX{src}, or vice versa). To fix this issue, we would
typically use locks to ensure that only one thread was updating \cTX{src} at a time; for example,

{\columnseprule=0.4pt

\begin{multicols}{2}
  \begin{Verbatim}
   // Send $5.00 from src to dst1
   lock(src);
   lock(dst1);
      src  = src - 5;
      dst1 = dst1 + 5;
   unlock(dst1);
   unlock(src);
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     // Send $10.00 from src to dst2
     lock(src);
     lock(dst2);
        src  = src - 10;
        dst2 = dst2 + 10;
     unlock(dst2);
     unlock(src);
\end{Verbatim}
\end{multicols}
}
\noindent (In \Java's monitor-based concurrency, we would use
a \cRW{synchronized} block rather than a \cTX{lock}/\cTX{unlock}
pair.) 

But programming with locks has a number of subtleties.
Looking at this particular pair of threads, it is very tempting to lock
just \cTX{src}; this would suffice to guarantee mutual exclusion,
and be faster.
But this would be a fragile optimization;
if a third thread wanted to access \cTX{dst1} or \cTX{dst2},
we would need to remember to come back and re-add locks here.
Even worse, to prevent deadlock (e.g., one thread locking \cTX{x} then
\cTX{y}, and a second locking \cTX{y} then \cTX{x}, and then both
deadlocking after acquiring one lock each) we might need a global
total order for acquiring locks. In this case, we might need to
acquire
locks for \cTX{dst1} and \cTX{src} in the opposite order, or 
(if references to accounts are indirect)
even do run-time tests to figure out the correct order in which to
lock accounts.

\subsection{Cooperative Multithreading}

The situation is significantly simpler under uniprocessor cooperative
multithreading.  Only one thread runs at a time, and we
switch between threads only when a thread terminates or explicitly
\yield{}s.  Since neither thread in the original code 
contains \yield, first one thread will run to completion
and then the other. Thus \cTX{src} will be reduced by a
total of \cTX{\$15}, without any need to specify locking. Our original
code is sufficient by itself:
{\columnseprule=0.4pt
\begin{multicols}{2}
  \begin{Verbatim}
   // Send $5.00 from src to dst1
   src  = src - 5;
   dst1 = dst1 + 5;
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     // Send $10.00 from src to dst2
     src  = src - 10;
     dst2 = dst2 + 10;
\end{Verbatim}
\end{multicols}
}

\iffalse
\cas{It's nice to have
a \yield example in the cooperative multithreading introduction. but 
I don't insist on including the following example; the discussion also
somewhat duplicates the discussion of the loop code below.}
\meo{I like it}
\fi

If other threads are permitted to view ``intermediate''
states where money has been removed from one account but not yet 
deposited into another, then we could instead write
{\columnseprule=0.4pt
\begin{multicols}{2}
  \begin{Verbatim}
   // Send $5.00 from src to dst1
   src  = src - 5;
   yield;
   dst1 = dst1 + 5;
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     // Send $10.00 from src to dst2
     src  = src - 10;
     yield;
     dst2 = dst2 + 10;
\end{Verbatim}
\end{multicols}
}
\noindent This version permits more possible schedules---for example, two decrements followed
by two increments, or the second thread running in its entirety
during the \yield of the first thread.
But even so, individual variable updates execute
without interruption, and ultimately \cTX{src} will decrease by
exactly \cTX{\$15}.   Crucially, the only reason that the
transfers can be interrupted in midstream is that the
programmer explicitly permitted it in the code.

A slightly more interesting example of cooperative multithreading
wraps the transfers
from our initial example in a
loop, sending money to both \cTX{dst1} and \cTX{dst2} until there is insufficient money left in \cTX{src} to perform any more transfers:
%\pagebreak
{\columnseprule=0.4pt

\begin{multicols}{2}
  \begin{Verbatim}
   while (src >= 5) {
      // Send $5.00 from src to dst1
      src  = src - 5;
      dst1 = dst1 + 5;

      yield;
   }
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     while (src >= 10) {
        // Send $10.00 from src to dst2
        src  = src - 10;
        dst2 = dst2 + 10;

        yield;
     }
\end{Verbatim}
\end{multicols}
}

\noindent Both loops include a call to \yield; otherwise one loop
would be forced to run in its entirety before the other loop got a
chance to run.  Not only is each update of \cTX{src} effectively
atomic, but the test and both update operations are atomic.  (The
exact sharing between \cTX{dst1} and \cTX{dst2} will depend on the
fairness of the scheduler.)  

\iffalse Further, both threads preserve
the total \cTX{src + dst1 + dst2} at each \yield point.  No third
observer thread will see an ``inconsistent'' state in which \cTX{src}
was decremented but \cTX{dst1} or \cTX{dst2} hadn't yet been
incremented to match.  \fi

We invite the reader to consider how one would write this trivial
example in traditional lock-based concurrency. This is 
trickier than it might appear, because one must 
prevent \cTX{src} from changing
between the test and following decrease.
Devising a solution with locks that doesn't
waste CPU time ``spinning'' or make it likely for one thread to starve
is even more challenging.\footnote{In the interests of implementation simplicity (c.f., correctness), on many real systems a loop that only releases a lock momentarily in an ``unlock then immediately relock'' sequence can starve other threads waiting for the lock.}

\subsection{Observationally Cooperative Multithreading (OCM)}

In OCM, we adopt the semantics of cooperative threading; we promise
that the observable behavior (i.e., input/output) of the system
remains the same as it would under uniprocessor cooperative threading,
but we expect to run multiple threads concurrently on many processors.  

In OCM, the fund-transfer code would change negligibly if disjoint accounts were being accessed,
{\columnseprule=0.4pt
\begin{multicols}{2}
  \begin{Verbatim}
   // Send $5.00 from src1 to dst1
   src1 = src1 - 5;
   dst1 = dst1 + 5;
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     // Send $10.00 from src2 to dst2
     src2 = src2 - 10;
     dst2 = dst2 + 10;
\end{Verbatim}
\end{multicols}
}
\noindent In contrast to conventional uniprocessor cooperative
multithreading, OCM can schedule these threads to run in parallel
because they access disjoint data---in the terminology of
\citet{Bernstein:66:anlyss-prgrms:itec}, they are
\emph{noninterfering}.
In many situations, most computation is noninterfering (either because an embarrassingly parallel divide and conquer solution is possible, or because different threads are doing unrelated things). In fact, some languages, such as \textsc{Cilk} 
\citep{Blumofe-et-al:95:clk-effcnt:ppopp},
% Which of many to cite, also Blumofe-et-al:96:clk-effcnt:jpdc, Randall:98:clk-effcnt:thesis
have parallel models where all parallel computation is expected to be
noninterfering.  

OCM does not require noninterference, because it can
(in the worst case) fall back to the behavior of uniprocessor
cooperative multithreading and run one thread at a time. But 
OCM can benefit in all the cases where noninterference exists.


\subsection{Atomic Blocks and Software Transactional Memory}

A popular research alternative to locks is the \atomic 
block~\citep{PeytonJones:07:btfl-cncrrncy:book}.  As the name suggests,
\atomic blocks guarantee that the enclosed code appears to execute
atomically, even in the presence of preemptive multitasking.

% So, we might write the original threads as
%{\columnseprule=0.4pt

%\begin{multicols}{2}
%  \begin{Verbatim}
%   // Send 5 units to dst1
%   atomic {
%      src = src - 5;
%      dst1 = dst1 + 5;
%   }
%  \end{Verbatim}
%\columnbreak
%\begin{Verbatim}
%     // Send 10 units to dst2
%     atomic {
%        src = src - 10;
%        dst2 = dst2 + 10;
%     }
%\end{Verbatim}
%\end{multicols}
%}
%\noindent to get the same effect of the lock-based code or the
%cooperative code.
Much as we used \cTX{lock}/\cTX{unlock} pairs or \Java
\cTX{synchronized} blocks around our simple example, in such a system
we would instead put the code inside an \atomic block. 
Atomic blocks are usually easier to use than locks.  With locks, we
must say what to lock, or which condition variable to wait on.
With \atomic blocks, there is nothing else to specify---the
implementation takes care of inferring data dependencies.


However, because of the block-structure of \atomic blocks, our
\cRW{while}-loop example is not so straightforward. Code
making the test and assignments atomic becomes
a bit convoluted; for example,
%\footnote{A similar approach can be used to ``solve'' the reader exercise from the previous section where we needed to support the loop with locks, although doing so does not address the spinning issue.}

{\columnseprule=0.4pt

\begin{multicols}{2}
  \begin{Verbatim}
   bool loop1;
   do {
      // Send $5.00 from src to dst1
      atomic {
         loop1 = src >= 5;
         if (loop1) {
            src  = src - 5;
            dst1 = dst1 + 5;
         }
      }
   } while(loop1);
  \end{Verbatim}

\columnbreak

\begin{Verbatim}
   bool loop2;
   do {
      // Send $10.00 from src to dst1
      atomic {
         loop2 = src >= 10;
         if (loop2) {
            src  = src - 10;
            dst1 = dst1 + 10;
         }
      }
   } while(loop2);
\end{Verbatim}
\end{multicols}
}



%\footnote{Interestingly, because of the static scoping of \atomic
%  blocks, they're not quite as convenient for simulating the
%  (cooperative) loop code. In the first thread, the test \cTX{src >=
%    5} and the assignment \cTX{src = src - 5;} needs to be in the same
%  atomic block (to prevent \cTX{src} from decreasing in the mean
%  time), but putting the entire loop inside an \atomic block would
%  severely restrict concurrency. But the code could presumably be
%  rewritten.} because they are more declarative (the programmer
%specifies what should be atomic, rather than how atomicity is to be
%guaranteed) and more compositional (atomic actions naturally combine
%into bigger atomic actions, whereas it can be tricky to properly
%combine two pieces of code that use locks.)

There are two typical approaches to implementing \atomic blocks. One
approach is for the system to automatically infer the correct locking actions
for each atomic block
\citep{Ringenburg-Grossman:05:atmcml-frstclss:icfp, Hindman-Grossman:06:atmcty-v:mspc,
  Emmi-et-al:07:lck-allctn:popl,Cherem-et-al:08:infrrng-lcks:pldi}. Research here largely focuses on
efficiency issues, such as finding the correct granularity for
assigning data to locks (e.g., one lock per array element to maximize
concurrency vs. one lock for the entire array to minimize the number
of lock operations).

The alternative approach for providing \atomic blocks (one that is increasingly popular among researchers and has been adopted by some newer languages such as Sun's Fortress~\citep{Allen-et-al:08:frtrss-lngg:tr}) is \keyterm{Software Transactional Memory}~\citep{Harris-et-al:05:cmpsbl-mmry:ppopp,Larus-Rajwar:07:trnsctnl-mmry:slca}.
Instead of
using locks, \atomic blocks are executed along the lines of
database transactions: if there is interference with another atomic
block, we roll back (undoing work) and reexecute the atomic
block. 

\iffalse
Most realizations of software transactional memory expose their transactional nature to the programmer, for example by providing a \retry operator that allows the current transaction to be voluntarily aborted aborted \citep{Harris-et-al:05:cmpsbl-mmry:ppopp}.
\fi

\section{\OCM vs Automatic Mutual Exclusion}


\keyterm{Automatic Mutual Exclusion}
(AME)~\citep{Isard-Birrell:07:atmtc-mtl:hotos,Abadi-et-al:08:smntcs-trnsctnl:popl} is a particularly relevant
variant of software transactional memory because of its parallels to
OCM. In fact, one way to view OCM is as a restricted form of AME. 

In traditional 
transactional memory, transactions are just blocks marked \atomic, and
only these blocks are synchronized; it is still possible to put too
little code inside an \atomic block. AME takes the safer but more
radical approach of assuming all code is atomic unless specifically
marked \unsynchronized.  AME atomic transactions are thus dynamically
delimited: the end of an atomic sequence is determined only at run time,
when control reaches an \unsynchronized block.


An empty \unsynchronized block in AME
dynamically ends one atomic block and begins another.  We could write our
earlier \cRW{while}-loop example in AME as:
{\columnseprule=0.4pt

\begin{multicols}{2}
  \begin{Verbatim}
   while (src >= 5) {
      // Send $5.00 from src to dst1
      src  = src - 5;
      dst1 = dst1 + 5;

      unsynchronized {
          // Empty
      }
   }
  \end{Verbatim}
\columnbreak
\begin{Verbatim}
     while (src >= 10) {
        // Send $10.00 from src to dst2
        src  = src - 10;
        dst2 = dst2 + 10;

        unsynchronized {
           // Empty
        }
     }
\end{Verbatim}
\end{multicols}
}

As one can see from this example, a \yield in OCM corresponds to an empty \unsynchronized block in AME.  This mapping immediately suggests an implementation technique for OCM---because we can view OCM as a subset of AME (where empty \unsynchronized blocks are the only AME facility used), we can use AME to provide an multiprocessor realization of OCM.


% \meo{I don't think we need this paragraph} The above loop is directly executable in AME with cooperative-multithreading
% semantics, even if the scheduler uses preemptive multitasking and
% executes the two threads on separate processors.  Each test and pair
% of assignments is implicitly atomic action; the underlying
% transactional memory implementation is responsible for detecting
% dynamic race conditions and rolling back one thread's atomic action if
% both loops try to update \cTX{src} at exactly the same instant.

\iffalse
Interestingly, there appears to be a small psychological distinction
between the implicit atomicity of OCM and the explicit declaration of
\atomic blocks.  All STM systems have some restrictions on what sort
of code can appear inside an \atomic block (forbidding thread
creation, or I/O, or other system calls).  The natural reaction is to
ask ``but why can't I have
\ldots in an atomic block''?  In contrast, in OCM you can create
threads or do I/O wherever you wants but these calls might
\yield; this feels less restrictive, even though it is
completely equivalent in practice.
\fi

AME differs from OCM in several respects, however.  Most notably, AME
requires an underlying implementation based on transactions and
rollback because of its \blockuntil operator.  This feature has similar
power to the \retry operator of \citet{Harris-et-al:05:cmpsbl-mmry:ppopp} that is present
in most systems providing software transactional memory. A \retry aborts
the current atomic transaction and retries it.  Providing a \retry operator does
increase expressiveness (e.g., the ability to automatically undo actions allows a
thread to \cTX{dequeue} from a
data structure and \retry if the resulting
value was not to its liking), but it also increases the complexity
of the language. More importantly, it requires the underlying
implementation to use transactions.  The cooperative-multithreading
programming model of OCM is simpler and is agnostic about the method
by which atomicity is guaranteed.

\iffalse
We believe that, by using a more sophisticated implementation
including, but not limited to, ideas from Transactional Memory and
lock inference (e.g., \citet{Emmi-et-al:07:lck-allctn:popl} and
\citet{Cherem-et-al:08:infrrng-lcks:pldi}), we can use multiprocessors to emulate
cooperative multithreading.  This would let programmers reason
according to the well-understood cooperative model---one thread
running at a time---but take advantage of true concurrency on
multiprocessors.  We call the resulting system \OCM (OCM).
\fi

\iffalse
AME's equivalent of the \retry operator is (somewhat misleadingly)
named \blockuntil (it would be better named \cTX{retryUnless}).  In AME, \blockuntil $p$ does \emph{not} \yield
until the condition $p$ becomes \cTX{true} and then continue on.
Instead, the AME semantics essentially rules out any execution order
(interleaving of thread actions) where the condition in a \blockuntil
evaluates to \cTX{false}. The only plausible way to implement this construct is
with transactions: execute code optimistically and test the condition
of \blockuntil at run-time; if it is \cTX{false}, then abort the
current atomic transaction, roll back to the start, and retry.

For example, assuming that we have a basic queue \cTX{q} supporting only
(atomic) \cTX{enqueue}, \cTX{dequeue}, and \cTX{isEmpty}
operations, the sequence

\begin{Verbatim}
    blockUntil (! q.isEmpty);
    a = q.dequeue();
    blockUntil (! q.isEmpty);
    b = q.dequeue();
    blockUntil (! q.isEmpty);
    c = q.dequeue();
\end{Verbatim}

\noindent will \emph{atomically} dequeue exactly three items from
\cTX{q}.  Furthermore, this sequence must wait to execute until
there are at least three items in the queue, so that all the
\blockuntil tests succeed.

Since the interface of \cTX{q} provides no way of checking in
advance that there are at least 3 items, locks and other mechanisms do
not suffice.  The only feasible way to implement this code atomically
is with transactions and rollback: try to dequeue three times, and
then ``undo'' these memory changes if the queue turns out to be empty
too soon.\footnote{Technically, the implementation could count items
  in the queue (without transactions) by dequeuing
  everything and then enqueuing everything, atomically. Not only would this be
  unacceptably slow, but it requires much more detailed knowledge of
  the semantics of queue operations than we can expect of a language
  implementation.} At some point later, we try again from the beginning.

\iffalse
\cas{Random thought: is there a sense in which this rollback would let
  one ``break'' abstractions?  Certainly \retry and \orelse could be
  used to test whether this simple queue has at least 3 elements.}
\fi

Because the base language of OCM is simply that of cooperative
multithreading, we lack this \blockuntil operator.\footnote {The
  original AME paper~\citep{Isard-Birrell:07:atmtc-mtl:hotos} mentions the possibility
  of requiring \blockuntil appear only at the beginning of atomic
  blocks, making it effectively a \cRW{yieldUntil} operator.  This
  would permit nonrollback implementations and \cRW{yieldUntil} is
  likely to be useful in OCM as well.  Later AME papers (e.g.,
  \citet{Abadi-et-al:08:smntcs-trnsctnl:popl, Abadi-Plotkin:09:mdl-cprtv:popl}) seem to have settled on the
  transactional approach, however.}  As a consequence, transactions
are certainly one way to implement the atomicity required for OCM, but
not the only way (e.g., \citet{Hindman-Grossman:06:atmcty-v:mspc}).  For example, one
might infer the locks required for atomic blocks; this might be
preferable for heavily shared pieces of memory, where conflicting
transactions repeatedly execute, rollback, and retry.
\fi

Further, OCM is in some senses ``safer'' than AME (or \atomic blocks).
Data access inside AME's \unsynchronized blocks is, by definition, 
data access without any protection against race conditions.
% (The \yield operation can be encoded as an \unsynchronized no-op.) 
Permitting synchronized code
% (\atomic blocks in traditional transactional memory; the default in AME) 
and unsynchronized code
% (default in traditional transactional memory; \unsynchronized blocks in AME)
to manipulate the same memory can lead
to unexpected behavior~\citep{Abadi-et-al:08:smntcs-trnsctnl:popl} under the more efficient
implementations of transactional memory.  It is possible to avoid
these effects with further language restrictions (e.g., a type system
dividing memory into locations accessible by atomic code and locations
accessible by unsynchronized code~\citep{Abadi-et-al:08:smntcs-trnsctnl:popl}, or a more
dynamic partitioning~\citep{Abadi-et-al:08:mdl-dynmc:concur}), but we would prefer to avoid the
issue entirely.


As a consequence of its design, the formal semantics of AME is
complex. In contrast, the semantics of
cooperative multithreading is simple: given a pool of threads,
execute one sequentially until it chooses to \yield; pick a new
thread from the pool; repeat.  

It may not be obvious how to construct an efficient
\emph{multi}processor implementation of OCM (or AME), but by looking
at cooperative multithreading, the intended semantics of OCM is
completely clear.  In contrast, the transactional-memory literature
contains various debates about proper behavior.  For example, what happens if
an exception is thrown in the middle of an atomic
block~\citep{Harris:05:excptns-sdffcts:socp}?
\begin{itemize}
\item  Should exceptions inside atomic blocks
be forbidden?
\item  Should we commit the transaction and continue to propagate the
  exception?
\item  Should we roll back and reexecute, hoping the 
  transaction will succeed on a second try?
\item Should we roll back but then
  propagate the exception?
\end{itemize}
%%% MEO: Was two paragraphs. I've joined them.

% CAS unjoined them, after edits to the previous paragraph

The AME papers are silent about exceptions, but the advantage of
starting with a simple high-level semantics for OCM is that it gives
clear guidance: if we want to simulate the behavior of exceptions in a
system of cooperative multithreading, then in OCM the exception ought to
propagate, and the exception handler should continue as an extension
of the same atomic block. 
%The handler may or may not choose to explicitly \yield.

Compared to AME, the possibility of nontransactional implementations,
or a hybrid approach involving both locks and rollback, can only
increase the chance of achieving acceptable performance and
scalability while maintaining ease of programming and reliability of
code.  We contend that the simpler cooperative-multithreading model of
OCM is sufficiently expressive for typical parallel programming tasks
and in fact can be easier to write for than AME.

\iffalse
It is likely that a \naive implementation of \OCM will have
high overhead and poor scalability. However, we hope that by avoiding
source-language features that force transactions and rollback, we have
more scope for optimization.
\fi

\section{Research Plans}

We propose to work on the following:
\begin{enumerate}
\item The design of OCM;
\item Implementation techniques for OCM;
\item Development of a full proof-of-concept implementation;
\item Construction of benchmarks making substantial use of OCM;
\item Measurement of the scalability, efficiency, and usability of OCM;
\item Formal semantics for OCM.
\end{enumerate}

We are well-positioned to conduct this inquiry.  Together we
are familiar with formal semantics; compiler implementation
from front-ends down to garbage collection; instrumentation and
analysis of concurrent programs; run-time techniques for detecting
interference between parallel tasks (determinacy checking); 
thread-scheduling algorithms; and the use of concurrency in real-world
systems code.

We anticipate that nine undergraduates (three each summer) will be
directly involved with the OCM design and implementation. A further six
(three each summer after the first) will be primarily involved
with OCM testing and benchmarking.

\subsection{Language Design}

At first glance the language design problem may seem trivial. If the
source language of OCM is just cooperative multithreading, it would
seem we just need to take the underlying sequential language and add
the minimal constructs for a typical user-level threads library (e.g.,
\citet{von-Behren-et-al:03:cprcc-sclbl:sosp}). These constructs would include \yield, a form of
\cTX{spawn} for creating new threads, and some sort of \cTX{exit} for
ending a thread.  

But a little thought suggests that, for reasons including convenience
and implementation efficiency, we may wish to extend the language
still further.  Examples include

\begin{enumerate}
\item There may be idioms that we wish to add as primitives.  For example, the polling-loop
  \begin{Verbatim}
    while (q.isEmpty) yield;
  \end{Verbatim}
could be replaced by a potentially more efficient primitive
\begin{Verbatim}
    yieldUntil (! q.isEmpty);
\end{Verbatim}
where, ideally, the thread would not be rescheduled until it has a
chance of succeeding.  

Similarly, using global variables and explicit
polling,  we could simulate the waking of a sleeping thread or the
killing of another thread.  But for both convenience and efficiency,
we might prefer these as primitives.

Alternatively, it may be better to provide only \yield and detect and optimize for these idioms both statically and dynamically.

\item When writing a subroutine, a key question becomes ``Should it
  \yield?'', and the answer may depend on the needs of the caller.
  Solutions are possible even with the basic OCM mechanisms (e.g., by
  adding a boolean \cTX{mayYield} argument to the function, forcing it
  to be atomic when needed and yielding otherwise to improve
  responsiveness). But there is a rich design space to explore to
  determine what level of support the OCM model itself should provide.

To give a flavor of the design space, we mention two avenues of interest:
\begin{enumerate}
\item Provide a notion of an adjustable \emph{scheduling context},
  where \yield only yields to threads in the current context.  To
  prevent a library function from yielding to other threads, we simply
  restrict the current context to contain only one thread.  Similarly,
  this approach might permit a notion of a computation that is atomic from the
  outside, but internally uses subthreads that \yield only to one another.

\item Describe a function's yielding behavior (won't \yield, could
  yield if context permits, might yield, definitely will yield, etc.)
  in its interface. \citet{Isard-Birrell:07:atmtc-mtl:hotos} sketched a design for AME
  in which functions were annotated to say whether they might \yield,
  and every call to such a function would be marked \yielding.
  Conversely, we could assume functions may yield unless specifically
  annotated (e.g., as \cTX{unyielding}).  In either case, 
  these annotations can be machine checked to
  make sure that they are correct~\citep{Talpin-Jouvelot:94:typ-effct:ic,Abadi:08:atmtc-mtl:unpub}.
\end{enumerate}

There are parallels between yielding and exceptions: yielding
specifications are clearly similar to exception specifications, and
scheduling context may be similar to exception-handler scope. Delimiting
the extent of these parallels may be a fruitful avenue of research.

\item Is it useful to be able to statically show that a function will
  eventually \yield?  In uniprocessor cooperative multithreading, a
  nonterminating thread that does not yield is inherently
  pathological.  In OCM, this pathology may be reduced (because we can
  make progress on other processors), but it may nevertheless be
  useful to know that a thread will \yield within a finite (or even
  exactly known) time; even an approximate analysis might be of
  use to the programmer for debugging.

\item Existing implementations of \atomic blocks often have strong
  restrictions on what can appear inside an \atomic block.  IBM's X10
  language has very strong restrictions, including ``the set of
  locations that are read and written \ldots are bounded and
  determined statically'' \citep{Saraswat-others:06:rprt-exprmntl:tr}.  Other transactional memory systems are
  more flexible, but usually forbid synchronous I/O and system calls;
  these cannot easily be rolled back. AME provides \unsynchronized
  blocks to permit such operations.

  We can largely sidestep this issue by declaring some library
  calls (e.g., those for doing I/O) as possibly \yielding. But
  we need to explore whether this approach is too restrictive in practice,
  and whether providing atomic versions of such calls
  \citep{Blundell-et-al:06:unrstrctd-trnsctnl:tr} might be feasible.
  
\iffalse
\meo{This is just a restatement of the above, I think}
\item In some code sequences, a \yield is unnecessary but harmless.
  For example, a function that spends time looping over purely local
  data could \yield every iteration, or every few iterations, to
  improve overall responsiveness of the system. But an explicit \yield
  would prevent the function from being called inside a larger atomic
  sequence.

  We would like to permit programmers to identify such points with a
  \maybeyield statement. We would then generate two pieces of code for
  functions involving \maybeyield: one that works atomically, and one
  that calls \yield.  If the static context of a function call
  suggests that the function needs to execute atomically (e.g., if the
  call is marked \atomic), then we would invoke the atomic version;
  otherwise, we might run the version that permits context-switching.
\fi

\iffalse
To extend the argument of \citet{Grossman:07:trnsctnl-mmry:oopsla} that
  atomic blocks and Transactional Memory are the concurrency
  equivalent of garbage collection for memory management, adding
  \maybeyield would be the equivalent of nulling-out pointers as hint
  to the garbage-collector.
\fi

\end{enumerate}


\subsection{Implementation Strategies}

There are a number of design choices for the core implementation of
OCM.  Each individual processor core might run threads cooperatively
(switching threads only on an explicit \yield) or preemptively
(interleaving computations on independent cooperative threads).
Further, there are a number of static and dynamic analyses that might
be necessary in practice.


\begin{enumerate}
\item Most obviously, we intend to experiment both with lock-based and
  transaction-based implementations of OCM atomic sequences. 

  We also suspect that not every atomic block needs to be
  implemented the same way.  Optimistic techniques (e.g., software transactional memory) might be
  better for data with ``low contention''.  Likewise, pessimistic
  techniques (e.g., locks) might be better for data with ``high contention''.


\item Any optimized implementation should statically determine which
  storage locations could be used by multiple threads and which are
  used only by a single thread; the latter need no special protection
  in atomic sequences.

\iffalse
\item \meo{Repetition. Already discussed in the previous section}
  It would be ideal if OCM programmers could call \yield only where it
  is necessary for correctness (e.g., within the producer's loop in a
  producer/consumer model), or implicitly via system calls (e.g.,
  input/output routines).  But the larger the atomic blocks, the more
  likely it is that blocks will want to manipulate the same data at
  the same time, leading to serialized execution or transaction
  rollbacks.

  Even better than having programmers specify
  \maybeyield points would be to have the system automatically infer where
  \maybeyield would be safe. We can use program analysis---perhaps
  even whole-program analysis, since it's a matter of optimization
  rather than correctness---to determine where it would be safe to \yield.
\fi

\iffalse
Nonterminating and nonyielding threads also causes difficulties for
automatically inserting \yield/\maybeyield. Assume we have a routine
that that modifies some global variables, loops over purely local
data, and then immediately yields.  If we know the loop terminates,
then it is safe to add an extra \yield inside the loop.  But if not,
then the code will never \yield after modifying the global variables;
it would be inconsistent with cooperative semantics for the rest of
the program to ever see these modifications.
\fi

\item By performing dynamic analyses (profiling), we can obtain
  information about how threads in specific programs tend to
  interact. We would like to feed this information back to the
  implementation (e.g., to choose whether optimistic or pessimistic
  synchronization is preferable for specific parts of the program,
  depending how often conflicts arise), and also back to the
  programmer (to suggest where serialization is occurring.).
  Techniques from feedback directed parallelism may be applicable
  here~\citep{Harris-Singh:07:fdbck-drctd:icfp}.
\end{enumerate}

We anticipate that our primary implementation will built the context
of a scripting language, such as Lua~\citep{Ierusalimschy-et-al:06:l-5:book} or Python~\citep{vanRossum-others:08:pythn-lngg:unpub}.

We see several
advantages to such an approach.  We can take advantage of existing
implementations with cooperative multithreading on uniprocessors
(e.g., Stackless Python~\citep{Tismer:00:cntntns-stcklss:unpub}). 
%Our first-year students have
%experience programming in Python. 
Additionally, we believe that users of scripting languages are most
likely to accept run-time overhead in return for an easy way to take
advantage of multiprocessors using an intuitive programming model.

Our goal is an OCM implementation that can be submitted and championed
through the necessary community processes for inclusion in subsequent
releases of the targeted scripting language.

\subsection{Benchmarking}

For \OCM to be successful, it must be both reasonably efficient and
scalable, and be relatively easy to use. In the second and third
years, we plan to hire three extra summer students specifically to
help evaluate our strategies for implementing OCM. We anticipate that these students will be
less-experienced undergraduates (e.g., between their first and second
year). Their success in writing benchmarks will thus provide further
qualitative evidence that OCM is an intuitive model for
programmers.  If the results are encouraging, we will encourage other 
groups at HMC to use OCM in their work.

On a quantitative basis, we are interested in looking at
\begin{enumerate}
\item The usual microbenchmarks; for example, cost of spawning new threads of
  control and other overheads involved in moving from sequential
  implementations to OCM;

\item Scalability and efficiency of OCM for larger benchmark programs
that do real work.  One possibility is to adapt existing code written
for cooperative concurrency, but other benchmarks should be
written specifically with OCM in mind.

% \meo{This looks like we're being evasive.}
% (In contrast, many larger transactional memory benchmarks were
% produced by taking existing code and replacing locks by atomic blocks;
% it is not clear this is the best comparison.  The use of locks can
% significantly affect how/what code is written; equivalent code written
% directly for transactional memory might be structured entirely
% differently, or use different data structures, or even support
% additional functionality.)
\end{enumerate}

In addition, providing feedback while developing benchmarks will
naturally get the undergraduates involved in the design and
implementation phases of the project.

\subsection{Formal Semantics}

It has long been understood how to formalize the meaning of a concurrent
imperative language using interleaving and a ``small-step'' operational
semantics~\citep{Hennessy-Plotkin:79:fll-abstrctn:mfcs}.
\iffalse (A denotational semantics of
cooperative
threads may not be so trivial
\citep{Abadi-Plotkin:09:mdl-cprtv:popl}, but this is not a goal of our work.)
\fi
Nevertheless, there are still interesting semantic questions,
including the following:

\begin{enumerate}
\item Can we use the formal semantics to justify correctness of the
  program analyses suggested above?

\item To implement OCM, we need to translate it into a lower-level
  language in which the mechanisms for implementing atomicity (e.g.,
  transactions, rollback, and locks) are exposed.  How can we define
  this language, and can we prove that the translation of OCM to this
  ``intermediate language'' preserves observational behavior? 


\item What fairness guarantees can we provide, and what should we
  expect? For example, consider a system that has useful threads, plus a
  thread that does nothing but loop without yielding.  In a
  cooperative system with a fair scheduler, this last thread would
  eventually run, and all progress would cease.

  In contrast, an OCM system might run this thread on one processor,
  and continue to schedule the other threads on other
  processors. This option can still be viewed as equivalent to a
  cooperative schedule, but an \emph{unfair} cooperative schedule in
  which the infinite-looping thread is not chosen until it is the
  only available thread.

We might be able to make stronger guarantees about fairness for
threads that eventually \yield. Exactly what guarantees are possible
is an interesting research question.

% \meo{Some options are (a) \yield = commit, or (b) certainty of
%   upcoming \yield means effects on the world can be allowed to
%   happen.}

\end{enumerate}

\section{Related Work: Threads and Events}

\iffalse
Similarly, the original ``double-checked locking
pattern'' (for initializing singleton objects) was widely recommended
for years before it was discovered to have a subtle race condition
under some legal implementations. And there is overhead in
automatically saving/restoring state on context switches, and in doing
the synchronization.
\fi

We are certainly not the first to observe that  the complexity of
synchronization can make it painfully
difficult to write concurrent code using common systems such as
\Pthreads or \Java threads \citep{Ousterhout:96:thrds-ar:unpub}. Reasoning
about locks---which locks must be acquired and when locks can be
released---quickly becomes complex and can depend on subtle
global invariants~\citep{Grossman:07:trnsctnl-mmry:oopsla}. 

A common alternative in systems code is event-driven programming:
threads are replaced by event handlers, scheduled by a central (and
sequential) dispatch loop.  Since only one handler runs at a time and
it runs until completion, there is little need for synchronization
between handlers and no context-switching overhead from
preemptions. This approach can be simple and efficient, but writing
complex code in an event-based form is not always natural.  In order
to maintain responsiveness, long-running tasks (e.g., those doing
blocking I/O) are split into many events that share a common
(heap-based) state. The result can be very similar to handwriting code in
continuation-passing style with hand-written closures.

An efficient nonpreemptive threading system might then be more
natural, and provide many of the synchronization advantages of events
\citep{von-Behren-et-al:03:evnts-ar:hotos,Gustafsson:05:thrds-wtht:queue}.  Some have pursued
more efficient implementations of cooperative
threading~\citep{von-Behren-et-al:03:cprcc-sclbl:sosp}, while others have compiled
thread-based source languages into an event-based
implementation~\citep{Fischer-et-al:07:tsks-lngg:pepm}.  There is still some debate about the
relative overheads of threads and events, but there is no doubt that
cooperative threads do provide an attractive and natural model for
systems programming.

However, cooperative threads and events both run one thread (or event)
at a time, and each must explicitly relinquish control to the next.
This approach can be fine for maximizing use of one processor, but a direct
implementation cannot take any advantage of a modern
multiprocessor. When true concurrency is desired, programmers have
tended to return to \Pthreads and similar preemptive systems, with all
the difficulties these schemes involve. We
see OCM as a promising alternative.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ocm"
%%% End: 


==> motivation.tex <==
%!TEX root = ocm.tex

\section{Motivation}

\meo{I think we have too much motivation.  I think we should push this material into the introduction, or into the concluding part of next section.}
The landscape of parallel computing is littered with attempts to finally make
parallel programming accessible to ordinary programmers. Much valuable progress
has been achieved, yet the models for parallelism in widespread use today are
still difficult for most programmers to use effectively. For example,
\citet{Rossbach-et-al:10:is-trnsctnl:ppopp} found that undergraduate students
in a systems class had more difficulty understanding the transactional
concurrency model than they did the coarse-grained locking model. However, when
they completed an assignment using both the locking and transactional models,
many more students made errors with explicit locking than with transactions.
From this we see that both the transactional and locking models have weaknesses
when it comes to ease of understanding and ease of use.  \goodbreak

Although locks and transactions have their advantages, better models are
necessary for parallel computing to prevail. \mjd{...against the evil ogre? This past sentence is weird and not entirely true. We're trying to make things better, parallel computing will prevail regardless.} We agree with
\citet{Skillicorn-Talia:98:mdls-lnggs:cmpsrv} that ``conscious human thinking
appears to us to be sequential, so that there is something appealing about
software that can be considered in a sequential way'', that ``models ought to
be as abstract and simple as possible'', and that ``[g]enerally, easy-to-use
tools with clear goals, even if minimal, are preferable to complex ones that
are difficult to use.'' By making a firm commitment to sequential cooperative
semantics, we believe that the OCM model makes significant progress towards
these goals.

%\cas{If we really cared about maximizing sequential reasoning, we'd use purely
%functional languages.  Do we have to explain why that's not our solution?}
%\jm{I think we want to build large desktop applications with GUIs like games,
%and do IO. }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% quotes

%``attacking the problem [of writing parallel programs] at the level of the model that acts
%as an interface between software and hardware issues.'' (126)

%``Generally, easy-to-use tools with clear goals, even if minimal, are
%preferable to complex ones that are difficult to use.'' (132)

%``conscious human thinking appears to us to be
%sequential, so that there is something appealing about software that can be
%considered in a sequential way.'' (125)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Past attempts


\iffalse
The landscape of parallel computing is littered with attempts to finally make
parallel programming accessible to ordinary programmers. Much valuable progress
has been achieved, yet the models for parallelism in widespread use today are
still difficult for most programmers to use effectively \cite{something}.
\amc{Do we really need another citation here? I've already added to the intro a
citation to support the claim that parallel programming is difficult.}

More than a decade ago, in their survey of parallel programming models,
Skillicorn \& Talia \cite{Skillicorn-Talia:98:mdls-lnggs:cmpsrv} outlined six important requirements for a
good parallel programming model. Two of these are that it be \emph{Easy to Use}
and \emph{Easy to Understand}. The main way to achieve this is by requiring the
programmer to wrestle with the details of his parallel program as little as
possible. They write, 

\begin{quote} As much as possible of the exact structure of the executing
program should be inserted by the translation mechanism (compiler and runtime
system) rather than by the programmer. (130) \end{quote}

Yet, in the years since Skillicorn \& Talia surveyed the
landscape of parallel-programming models, we still see the difficulties
associated with the fact that today's models are not sufficiently easy to use
or understand.

We believe that for parallel computing to prevail, we need models that address
these concerns better than the models for multicore computing that are
available to mainstream programmers today.  As simple as locks and STM are, a
model which completely abstracts away the implementation of collision control
adheres more closely to the requirements laid out by Skillicorn \& Talia, fulfilling 
their advice that ``models ought to be as abstract and simple as possible.'' (130).  
Observationally cooperative multithreading is our attempt at providing such a 
model.
\fi

\iffalse
More than a decade ago, in their survey of parallel programming models,
Skillicorn \& Talia \cite{Skillicorn-Talia:98:mdls-lnggs:cmpsrv} outlined six important requirements for a
good parallel programming model. Two of these are that it be \emph{Easy to Use}
and \emph{Easy to Understand}. The main way to achieve this is by requiring the
programmer to wrestle with the details of his parallel program as little as
possible. They write, 

\begin{quote} As much as possible of the exact structure of the executing
program should be inserted by the translation mechanism (compiler and runtime
system) rather than by the programmer. (130) \end{quote}

Yet, in the years since Skillicorn \& Talia surveyed the
landscape of parallel-programming models, we still see the difficulties
associated with the fact that today's models are not sufficiently easy to use
or understand.
\fi

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ocm"
%%% End: 

%!TEX root = ocm.tex



==> relatedwork-alt.tex <==
%!TEX root = ocm.tex

\section{Related Work}
\label{sect:related}

As a parallel model, OCM intersects with a significant portion of prior work on
parallelism and concurrency. There is a vast literature describing parallel
models, concurrency-control mechanisms, debugging techniques, and so forth that
could be related to OCM, but to which we cannot hope to do justice in the space
available. Thus, we must restrict our discussion to those techniques that we feel are
of most interest because they parallel, influence, or counterpoint OCM in some
way. 

\subsection{Other Models of Concurrency}
 \label{sect:related-ame}
 There are, of course, many other models for parallel programming
 besides those discussed in
 Section~\ref{sect:issues-with-existing-models}, including
 monitors~\cite{Hoare:74:monitors:cacm} 
%and Java \synchronized
% methods~\cite{Gosling:05:JLS:book}, 
 communicating sequential
 processes~\cite{Hoare:85:CSP:book}, 
%Threading Building Blocks~\cite{Reinders:07:TBB:book}, 
 and
 OpenMP~\cite{OpenMP:08:OpenMPAPI3.0:spec}, to name just a few.  
% Many
% of these were also intended to be simple and/or permit sequential
% reasoning in the presence of concurrency.  
 We cannot compare each in detail here, but to the extent that they provide
 particular scheduling policies or ways to create new threads
 (e.g., parallel \cRW{for} loops), they may be transferrable to an OCM
 context. However, two further models deserve specific comparison with
 OCM.

\paragraph{Automatic Mutual Exclusion}
 AME~\cite{Isard-Birrell:07:atmtc-mtl:hotos,Abadi-et-al:08:smntcs-trnsctnl:popl}
 is a variant of software transactional memory.  Rather than starting
 with unsynchronized code and marking particular blocks as \atomic,
 AME makes the safer assumption that all code should
 be executed atomically unless specifically marked
 \unprotected. Consequently, atomic code is dynamically delimited by
 the execution of \unprotected blocks.  An AME system could 
 easily be used to implement OCM (\yield corresponds to an empty
 \unprotected block~\cite{Abadi-et-al:08:smntcs-trnsctnl:popl}), 
 and AME has already engendered work on the denotational semantics of
 uniprocessor cooperative multithreading~\cite{Abadi-Plotkin:09:mdl-cprtv:popl}.

 While we have found the AME work inspiring, there are two important
 ways in which OCM intentionally differs from AME.  Both follow
 naturally from CM serializability, but we believe the differences
 also make OCM both simpler and safer.

 First, AME is explicitly transaction-based. Its
 \blockuntil operator permits users to roll back and retry
 transactions, allowing code that is impossible without 
 transactions to track and undo side-effects. In contrast,
 OCM has multiple implementations, including lock-based 
 schemes that can be more efficient for some programs.

 Second, OCM has no escape hatch for ``lower-level'' memory operations
 outside of OCM's concurrency-control system. Non-empty \unprotected
 blocks can improve performance, but they can also be a
 source of bugs and semantic
 surprise~\cite{Shpeisman-et-al:07:enfrcng-isltn:pldi}.

% \meo{We hark back to non-parallel CM, Cilk also harks back to non-parallel C.
% Also, many Cilk programs could be OCM programs that don't really need to yield.}

\paragraph{Cilk}
Cilk~\cite{Blumofe-et-al:95:clk-effcnt:ppopp,Frigo-et-al:98:implmnttn-clk5:pldi98}
 is a parallel extension of C.
Although it largely relies on the programmer to prevent interference
between threads, it is interesting to compare Cilk's \keyterm{serial
  elision} property with CM serializability. 

Serial elision
guarantees that Cilk keywords can be omitted---replacing 
\cRW{spawn}ed function calls with ordinary function calls,
and removing all \cRW{sync} barriers---to obtain a legal C program with
the same semantics as the Cilk version running on one processor.
The Cilk version running on a multiprocessor may produce
additional behaviors (due to race conditions and other
nondeterminism).

The CM serializability guarantee goes in the opposite direction:
the behaviors of OCM running on a multiprocessor cannot exceed
the possible behaviors from a uniprocessor CM implementation.

\iffalse
% No room, I think
We speculate that there is an even more direct link between the two
systems: code written to the Cilk model has no contention 
between threads, and thus should be should not be difficult to
port to the OCM model: OCM handles contention between threads, but
in principle should be equally happy if no contention exists.
\fi

\subsection{Methods for Reducing OCM Overhead}
 \label{sect:ocm-overhead}
 \label{sect:related-lockinf}

There are many ways to implement OCM. For example, OCM can use a pessimistic lock-based approach. 
\keyterm{Lock Inference} is a method for the system to infer the correct locking actions
automatically \cite{Ringenburg-Grossman:05:atmcml-frstclss:icfp,
  Hindman-Grossman:06:atmcty-v:mspc,
  Emmi-et-al:07:lck-allctn:popl,Cherem-et-al:08:infrrng-lcks:pldi,KhilanGudka:10:hll-wrld:tr}. 
%Research here largely
%focuses on efficiency and accuracy issues
%, such as finding the correct granularity
%for assigning data to locks (e.g., one lock per array element to
%maximize concurrency vs. one lock for the entire array to minimize the
%number of lock operations), or scaling to large code bases.
Research advances in lock inference can be directly applied to
lock-based OCM implementations.

 \label{sect:related-stm}
 There is also significant ongoing research into \keyterm{Software Transactional
  Memory}~\cite{Shavit-Touitou:95:sftwr-trnsctnl:podc,Larus-Rajwar:07:trnsctnl-mmry:slca,Spear:10:lghtwght-rbst:spaa}
(and even hardware support for transactional memory~\cite{Harris-et-al:05:cmpsbl-mmry:ppopp,Larus-Rajwar:07:trnsctnl-mmry:slca}). STM
 has even been adopted by some
newer languages such as Sun's
Fortress~\cite{Allen-et-al:08:frtrss-lngg:tr}.
Switching an STM-based OCM implementation from one STM library
to another is not
difficult, as long as the STM interfaces are reasonably similar. As a
result, an STM-based OCM implementation
can choose the STM implementation with the best performance
characteristics.

In general, implementation advances in other models of concurrency 
should permit improved implementations of OCM.
\iffalse
, and OCM can benefit from performance improvements to the underlying STM
implementation without any further modifications.  STM implementations continue
to improve, and a current area of active research is techniques for dynamically
adapting an STM implementation based on the current behavior of the executing
program~\cite{
\fi

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ocm"
%%% End: 


==> semantics.tex <==
%!TEX root = ocm.tex

% \section{Semantics}

\iffalse
The OCM model adopts the syntax and semantics of Cooperative
Multithreading, and so to discuss the semantics of OCM we first
must clarify our interpretation of CM.

\subsection{Cooperative Multithreading}

Given a sequential language, we can extend it to Cooperative
Multithreading by adding two operations: \yield and \spawn. Instead
of single thread of control running sequentially, a CM
program consists of a collection of such threads of control; initially
there is just the main thread, but each use of \spawn adds a new
thread to the collection. During the lifetime of the program, exactly
one thread is executing at a time: the system repeatedly picks a
available thread and runs it (following the semantics of the
underlying sequential language) until that thread voluntarily yields
or terminates.

Note that we do not specify a particular scheduling algorithm. In
particular, the thread that \yield{}s might immediately resume
execution, even if other threads are available.  However, we add one
very weak fairness assumption for any reasonable CM implementation: in
the absence of ``uncooperative'' threads that execute forever without
terminating or \yield{}ing, we guarantee that any thread that
\yield{}s will eventually be picked to resume execution.  Conversely,
in the presence of uncooperative threads, then some thread or threads
might never resume.
 
Another way to view the turn-taking of the cooperative threads by viewing
the code between dynamically successive \yield{}s as a critical
section. We can thus recast the properties of CM as the usual
properties of critical sections, including mutual exclusion
(i.e., only one thread executing at a time), progress (i.e., when a
thread yields some thread will begin executing), and bounded waiting
(i.e., that a thread waiting to resume will eventually be picked to
execute).  \cas{eventually $\ne$ bounded. Do we want to require
bounded for any OCM implementation?}
\fi % \iffalse


\iffalse
It is instructive to consider the possibility of an ``uncooperative'' thread
that executes forever without terminating or \yield{}ing. In the
absence of ill-behaved threads, every thread that \yield{}s will 
eventually resume. 

Ill-behaved threads cannot violate our fairness/bounded waiting
assumption. Even provably bounded-waiting algorithms for critical
sections, such as XXX, provide no help if a process refuses to leave a
critical section.  Similarly, if our ill-behaved thread never yields,
then we never again have the opportunity to resume other waiting
threads and thus we do not have the opportunity to be unfair to them.
\fi

\iffalse
\subsection{Observationally Cooperative Multithreading}

The correctness criterion for an OCM implementation is that the
\emph{observable} behavior (final results, I/O, etc.) of a program run
under OCM will be consistent with some possible execution under a
nonpreemptive uniprocessor CM model. 



For those programmers more familiar with the use of traditional
preemptive mechanisms, we can give an alternative characterization:
the computations between any two dynamically successive \yield{}s
execute atomically. \cas{Forward reference AME here?}  That is, the
concurrent implementation is linearizable with respect to computations
between \yield{}s.

Consequently, threads behave as if completely isolated from each other
except at \yield points. This provides a useful characterization for
guiding the placement of \yield{}s: a \yield
statement is where a thread publishes its changes to the surrounding
environment, and where it receives other threads' changes to that
environment.

\bigskip Since OCM behavior must remain consistent with CM, in the
absence of uncooperative non-yielding threads, any OCM implementation
will also satisfy the constraint that all threads that yield will
resume. \cas{In a bounded number of system yields?}.

Now in a typical uniprocessor implementation of CM,
once the uncooperative thread begins execution it will never yield,
and hence all other threads will be blocked.

This might occur in OCM implementations as well. But depending on the
OCM implementation and whether the uncooperative thread is using only
unshared data, it is possible that the uncooperative thread might run
forever on one processor (unobservably, since it never yields), while
other processors execute the remaining thread to perform observable
useful work.  This is explainable only in terms of a CM linearization
in which the uncooperative thread is never picked to execute. 

Thus, we were intentially careful in defining the CM model to say that
in the presence of uncooperative threads, \emph{some} thread or threads
might never be picked to resume.  


\fi

\iffalse
Cooperative multithreading has many advantages. It allows simple
reasoning: between \yield{}s we can reason about code as if it were
purely sequential. Because we know no other code is running until we
choose to yield, we can often avoid the complexity and runtime
overhead of locks and other protection mechanisms.


That is, it promises that the observable behavior of a program written
in the OCM model and executed with an OCM system will be the same as
if it were run using a CM system, except that it will (hopefully) run
faster. That's because, unlike CM, OCM typically takes advantage of
concurrency-control mechanism.  But, by adopting the CM semantics, OCM
also guarantees serializability. That is, an OCM system \emph{could}
be written with an underling implementation which simply executes code
serially, or the same effect could be achieved by running an OCM
program with a typical OCM system on a single processor. Regardless,
the program execution is guaranteed to be equivalent, saving the
effects of indeterminism and race conditions.
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ocm"
%%% End: 

